Inverse regression for ridge recovery: A data-driven approach for parameter reduction in computer experiments

Parameter reduction can enable otherwise infeasible design and uncertainty studies with modern computational science models that contain several input parameters. In statistical regression, techniques for sufficient dimension reduction (SDR) use data to reduce the predictor dimension of a regression problem. A computational scientist hoping to use SDR for parameter reduction encounters a problem: a computer prediction is best represented by a deterministic function of the inputs, so data comprised of computer simulation queries fail to satisfy the SDR assumptions. To address this problem, we interpret SDR methods sliced inverse regression (SIR) and sliced average variance estimation (SAVE) as estimating the directions of a ridge function, which is a composition of a low-dimensional linear transformation with a nonlinear function. Within this interpretation, SIR and SAVE estimate matrices of integrals whose column spaces are contained in the ridge directions' span; we analyze and numerically verify convergence of these column spaces as the number of computer model queries increases. Moreover, we show example functions that are not ridge functions but whose inverse conditional moment matrices are low-rank. Consequently, the computational scientist should beware when using SIR and SAVE for parameter reduction, since SIR and SAVE may mistakenly suggest that truly important directions are unimportant.

==> sec1-intro-pc.tex <==
% Inverse regression as ridge recovery: a data-driven approach for parameter space dimension reduction in computational science models

\section{Introduction and related literature}
\label{sec:intro}















Data science and machine learning methods are essential tools in modern data-driven computational science and engineering. The computational scientist frequently uses supervised learning techniques (i.e., curve fitting) to identify trends, quantify uncertainty, predict unobserved phenomena, and optimize engineered designs in complex physical systems. The most commonly used supervised learning approaches include methods for regression modeling (as opposed to classification), since both input features and output quantities of interest are best modeled as continuous real variables. 
These approaches appear under several names: response surfaces~\cite{Myers1995,Jones2001}, surrogate models~\cite{Razavi2012,Allaire2010}, metamodels~\cite{Wang2006}, and emulators~\cite{Challenor2012}; we use the term \emph{response surface} in the remainder. 

We generically model a physics-based input/output system as a function $f(\vx)$, where $\vx$ represents a vector of continuous physical inputs and $f$ represents a continuous physical output of interest. It is common to treat $f$ as a deterministic function, since a bug-free computational model produces the same outputs given the same inputs; in other words, there is no random noise in simulation outputs. This perspective is the de facto setup in the statistics subfield of \emph{computer experiments}~\cite{Sacks89,Koehler96,Santner03}, where Gaussian process regression~\cite{gpml2006} is the supervised learning tool of choice. The setup is similar in the field of \emph{uncertainty quantification}~\cite{SmithUQ2013,SullivanUQ2015,HandbookUQ}; although the inputs may be modeled as random variables to represent aleatory uncertainty, the input/output map is deterministic. 

Several important, oft overlooked mathematical challenges arise when applying regression methods to a dataset comprised of point queries of a deterministic function. In regression modeling~\cite{Weisberg2005}, the given data are predictor/response pairs $\{(\vx_i, y_i)\}$ that are assumed to be independent realizations of a random vector with a joint predictor/response probability density function. If the response is a deterministic function of the predictors, then such a density cannot exist. Thus, the data from computational science simulations fail to satisfy the regression assumptions. This failure has important consequences for interpreting \emph{error} and \emph{convergence} in the response surface. We do not explore these consequences in this paper, but the differences between statistical regression and function approximation are essential to our thesis. 

Nonparametric regression approaches are most appropriate for computational science data since the physical complexities produce nonlinear responses. However, the nonlinearity implies that response surface construction suffers from the \emph{curse of dimensionality}~\cite{Donoho00,Traub1998}; loosely, the number of function queries needed to construct an accurate response surface grows exponentially with the input predictor dimension. In computational science, this curse is exacerbated by the computational cost of each query, which often involves the numerical approximation of a system of partial differential equations. In high dimensions (i.e., several physical input parameters), the number of queries needed to reach error estimate asymptopia (or even construct the response surface) is generally considered infeasible. The computational scientist may attempt to simplify the model by fixing unimportant input parameters at nominal values, thus reducing the dimension of the input space to the point that response surface modeling becomes practical. 

Both linear~\cite{Cunningham2015} and nonlinear~\cite{Lee2007} dimension reduction methods are well known in unsupervised learning, and they are appropriate for computational science input parameter spaces when there is a relationship (e.g., correlation structure) among the input parameters. However, in many cases the physical inputs are independent. Therefore we must use dimension reduction approaches, such as active subspaces~\cite{Constantine15}, that are derived from low-dimensional structure in the input/output map. 

In regression modeling, subspace-based predictor space dimension reduction goes by the name \emph{sufficient dimension reduction} (SDR)~\cite{Cook98,Adragni09}. Techniques for SDR include sliced inverse regression (SIR)~\cite{Li91}, sliced average variance estimation (SAVE)~\cite{Cook91}, ordinary least squares (OLS)~\cite{OLS89}, and principal Hessian directions (pHd)~\cite{Li92}---among several others. These techniques seek a low-dimensional subspace in the predictor space that is sufficient to statistically characterize the relationship between predictors and response. Related techniques and extensions have enabled feature space dimension reduction in supervised learning models~\cite{Mukherjee2010,Wu2010,Fukumizu2014}. And SDR methods are gaining interest for parameter space dimension reduction in computational science~\cite{Li16,Zhang2017,Pan2017}. The first use we know applies OLS, SIR, and pHd to a contaminant transport model from Los Alamos National Labs, where the results revealed simple, exploitable relationships between transformed inputs and the computational model's output~\cite[Section 4]{Cook94b}. However, these papers do not carefully address the important mathematical differences that arise when applying a technique developed for statistical regression to study a deterministic function. A data set comprised of point queries from a deterministic function (e.g., an experimental design in the physical inputs and associated computer model predictions) differs from the regression data set (independent draws of a joint predictor/response distribution). How does one interpret a dimension reduction subspace from SIR or SAVE when there is no random noise in the functional relationship between inputs and outputs? What does \emph{sufficient dimension reduction} mean for deterministic functions?

We evaluate and analyze the \emph{inverse regression} methods SIR and SAVE as candidates for gradient-free subspace-based input space dimension reduction in deterministic functions. SIR- and SAVE-style dimension reduction follows from low-rank structure in the regression's inverse conditional moment matrices. The appropriate way to interpret SIR and SAVE in this context is as methods for \emph{ridge recovery}. A function of several variables is a \emph{ridge function} when it is a composition of a low-dimensional linear transformation with a nonlinear function of the transformed variables~\cite{Pinkus15}---i.e., $f(\vx)=g(\mA^\top\vx)$ where $\mA$ is a tall matrix. The goal of ridge recovery is to estimate the matrix $\mA$ (more precisely, $\mA$'s column space known as the \emph{ridge subspace}) using only point queries of $f$. Recent work by Fornasier, Schnass, and Vybiral~\cite{Fornaiser12} and related work by Tyagi and Cevher~\cite{Tyagi2014} develop ridge recovery algorithms that exploit a connection between a linear measurement of a gradient vector and the function's directional derivative to estimate $\mA$ with finite differences. Constantine, Eftekhari, and Wakin~\cite{constantine2015sketching} exploit a similar connection to estimate active subspaces with directional finite differences. In contrast, the inverse regression approach for ridge recovery is based on conditional moments of the predictors given the response; we detail how this difference (gradients versus inverse conditional moments) affects the methods' ability to recover the ridge directions. 

\subsection{Main results and discussion}
We develop and interpret sufficient dimension reduction theory in the context of input space dimension reduction for a deterministic scalar-valued function of several variables. By this interpretation, SDR methods translate naturally as ridge recovery methods; loosely, the noiseless analog of SDR is ridge recovery. 
This interpretation illuminates the theoretical limitations of inverse regression for parameter space dimension reduction. We show that, if the data-generating function is a ridge function, then the population (i.e., no error from finite sampling) SIR and SAVE subspaces are (possibly strict) subspaces of the function's ridge subspace. Consequently, the rank of the inverse conditional moment matrices is bounded above by the dimension of the ridge subspace. We also show how the inverse conditional moments become integrals, so that the finite-sample SIR and SAVE algorithms can be viewed as numerical integration methods. By choosing input samples independently at random, SIR and SAVE become Monte Carlo methods; we analyze the convergence of SIR and SAVE subspaces as the number $N$ of samples increases and derive the expected $\mathcal{O}_p(N^{-1/2})$ rate, where $\mathcal{O}_p$ denotes convergence in probability and the constant depends inversely on associated eigenvalue gap. Moreover, this view enables more efficient numerical integration methods than Monte Carlo for SIR and SAVE~\cite{Glaws2018}.

\subsection{Practical considerations and scope}
Some readers want to know how these results impact practice before (or in lieu of) digesting the mathematical analysis. In practice, the computational scientist does not know whether her model's input/output map is a ridge function, and she'd like to use SIR and SAVE as a tool to test for possible dimension reduction; our theory gives some insight into this use case. First, in the idealized case of no finite-sampling (or numerical integration) error, SIR and SAVE can still mislead the practitioner, since there are non-ridge functions whose inverse conditional moment matrices are low-rank. Arguably, these may be pathological cases that do not arise (frequently) in practice, but quantifying this argument requires mathematically characterizing a \emph{typical problem} found in practice. We believe these failure modes should be well known and guarded against. Second, finite sample estimates (or numerical approximations) of the inverse conditional moment matrices will never have trailing eigenvalues that are exactly zero due to the finite sampling---even when the data-generating function is an exact ridge functions. This implies it may be difficult to distinguish between finite-sample noise in the eigenvalues and directions of small-but-nonzero variability in the function. The latter structure indicates anisotropic parameter dependence that is arguably more common in real world functions than exact ridge functions, and it (the anisotropy) can be exploited for ridge approximation (as opposed to ridge recovery). Because of such indistinguishability, we recommend exercising caution when using the estimated SIR and SAVE subspaces to build ridge approximations. Principally, heuristics such as bootstrapping or cross validation might help distinguish between finite sample noise and directions of relatively small variability. Third, we have found that breaking the elliptic symmetry assumption on the input density (see Section \ref{subsec:SIR})---e.g., when the input density is uniform on a hyperrectangle---may produce nonzero eigenvalues in the inverse conditional moment matrices even when the data-generating function is an exact ridge function; distinguishing these effects from finite-sample effects or true variability in the data-generating function may be difficult. All these issues, though important in practice, are outside the scope of the present work. However, we do make some comments on practical considerations in the numerical example in Section \ref{subsec:hartmann}.

\subsection{Paper outline}
The remainder is structured as follows. Section \ref{sec:SDR} reviews (i) the essential theory of sufficient dimension reduction in statistical regression and (ii) the SIR and SAVE algorithms. In Section \ref{sec:ridge_funcs}, we review ridge functions and the ridge recovery problem. Section \ref{sec:SDR_for_RR} translates SDR to deterministic ridge recovery and analyzes the convergence of the SIR and SAVE subspaces. Section \ref{sec:numericalresults} shows numerical examples that support the analyses using (i) two quadratic functions of ten variables and (ii) a simplified model of magnetohydrodynamics with five input parameters. Section \ref{sec:conclusion} contains concluding remarks. To improve readability, all proofs are in the Appendix.


